How Well Do Large Language Models Truly Ground?

To reduce issues like hallucinations and lack of control in Large Language Models (LLMs), a common method is to generate responses by grounding on external contexts given as input, known as knowledge-augmented models. However, previous research often narrowly defines "grounding" as just having the correct answer, which does not ensure the reliability of the entire response. To overcome this, we propose a stricter definition of grounding: a model is truly grounded if it (1) fully utilizes the necessary knowledge from the provided context, and (2) stays within the limits of that knowledge. We introduce a new dataset and a grounding metric to evaluate model capability under the definition. We perform experiments across 25 LLMs of different sizes and training methods and provide insights into factors that influence grounding performance. Our findings contribute to a better understanding of how to improve grounding capabilities and suggest an area of improvement toward more reliable and controllable LLM applications.

==> emnlp2023-latex/prompts.tex <==
\onecolumn
\lstset{%
  language=[LaTeX]TeX,
  backgroundcolor=\color{gray!25},
  basicstyle=\ttfamily,
  breaklines=true,
  breakindent=0pt,
  columns=fullflexible
}

\begin{lstlisting}[caption={Prompt for NQ natural form}, label=NNF,captionpos=b]
Generate an [Explanation] for the [Answer] of the [Question] based on only the given facts from [Supporting Documents]. Any content of [Explanation] brought from [Supporting Documents] should have exactly matching spans of text.


[Question]
who played smiley in tinker tailor soldier spy

[Answer]
Gary Oldman

[Supporting Documents]
#1. [Tinker Tailor Soldier Spy (film)]
 Tinker Tailor Soldier Spy is a 2011 Cold War spy thriller film directed by Tomas Alfredson.
 The screenplay was written by Bridget O'Connor and Peter Straughan, based on John le Carré's 1974 novel of the same name.
 The film, starring Gary Oldman as George Smiley, along with Colin Firth, Tom Hardy, John Hurt, Toby Jones, Mark Strong, Benedict Cumberbatch, and Ciarán Hinds, and featuring David Dencik, is set in London in the early 1970s and follows the hunt for a Soviet double agent at the top of the British secret service.

[Explanation]
Direct evidence is provided by [#1 Tinker Tailor Soldier Spy (film) : The film, starring Gary Oldman as George Smiley] stating that Gary Oldman played smiley in tinker tailor soldier spy. So the answer is Gary Oldman.


[Question]
how many power rangers series has tommy been in

[Answer]
five

[Supporting Documents]
#1. [Tommy Oliver]
 According to the character's history, Tommy is a legend among the Power Rangers community and is considered to be the greatest Power Ranger of all time, having been five different Power Rangers — the Green Ranger, the White Ranger, Zeo Ranger V–Red, the Red Turbo Ranger, and the Dino Thunder Black Ranger — and a part of four Ranger teams over the years.
 In addition, Tommy is a lifelong practitioner of the martial arts; during the first season of "Power Rangers", he was referred to as having a third-degree black belt in karate.
 By "Power Rangers Dino Thunder", he is a 6th degree black belt. ("
 Return of the Ranger", "Power Rangers Dino Thunder – Collision Course" DVD).
 Tommy also serves as a love interest to the original Pink Ranger Kimberly Hart before their separation.
 He later pursued a relationship with Kimberly's successor Kat Hillard.
 
[Explanation]
[#1 Tommy Oliver : considered to be the greatest Power Ranger of all time, having been five different Power Rangers] states that tommy has been in five power rangers series. So the answer is five.


[Question]
what is the name of the sea surrounding dubai

[Answer]
Persian Gulf

[Supporting Documents]
#1. [Dubai]
 Dubai ( ; "", ) is the largest and most populous city in the United Arab Emirates (UAE).
 On the southeast coast of the Persian Gulf, it is the capital of the Emirate of Dubai, one of the seven emirates that make up the country.

[Explanation]
Based on a document about dubai, [#1 Dubai : On the southeast coast of the Persian Gulf, it is the capital of the Emirate of Dubai], the name of the sea surrounding dubai is Persian Gulf. So the answer is Persian Gulf.


[Question]
when did the movie deuces come out

[Answer]
2017

[Supporting Documents]
#1. [Deuces (film)]
 Deuces is an American crime drama written and directed by Jamal Hill.
 The film stars Larenz Tate, Meagan Good, Lance Gross and Siya.
 The film is executive produced by Queen Latifah for her production company Flavor Unit Entertainment. "
 Deuces" premiered on Netflix on April 1, 2017.

[Explanation]
Information related to deuces is shown in [#1 Deuces (film) : "Deuces" premiered on Netflix on April 1, 2017.]. the movie deuces came out in 2017. So the answer is 2017.


[Question]
why do leaflets of mimosa fold when touched

[Answer]
defending themselves from harm

[Supporting Documents]
#1. [Mimosa pudica]
 Mimosa pudica (from "shy, bashful or shrinking"; also called sensitive plant, sleepy plant, action plant, Dormilones, touch-me-not, shameplant, zombie plant, or shy plant) is a creeping annual or perennial flowering plant of the pea/legume family Fabaceae and Magnoliopsida taxon, often grown for its curiosity value: the compound leaves fold inward and droop when touched or shaken, defending themselves from harm, and re-open a few minutes later.
 In the UK it has gained the Royal Horticultural Society's Award of Garden Merit.

[Explanation]
A particular document abput mimosa's, [#1 Mimosa pudica : the compound leaves fold inward and droop when touched or shaken, defending themselves from harm] explains that leaflets of mimosa fold when touched for defending themselves from harm. So the answer is defending themselves from harm.
\end{lstlisting}


\begin{lstlisting}[caption={Prompt for HotpotQA natural form}, label=HNF,captionpos=b]
Generate an [Explanation] for the [Answer] of the [Question] based on only the given facts from [Supporting Documents] . Any content of [Explanation] brought from [Supporting Documents] should have exactly matching spans of text.



[Question]
Were Scott Derrickson and Ed Wood of the same nationality?

[Answer]
yes

[Supporting Documents]
#1. [Scott Derrickson]
  Scott Derrickson (born July 16, 1966) is an American film director, producer, and screenwriter.
  He lives in Los Angeles, California.
  Derrickson is best known for directing horror film, "Sinister" (2012), and as well as the Marvel Cinematic Universe superhero film "Doctor Strange" (2016).
#2. [Ed Wood]
  Edward Davis Wood Jr. (October 10, 1924 – December 10, 1978) was an American filmmaker, actor, and author.

[Explanation]
Derrickson was [#1 Scott Derrickson : an American film director, producer, and screenwriter.], while Wood was [#2 Ed Wood : an American filmmaker, actor, and author.]. Both Scott Derrickson and Ed Wood were American filmmakers, so they share the same nationality. So the answer is yes.


[Question]
Martin Patterson "Pat" Hingle was a close friend of an actor who achieved success in what Western TV series? 

[Answer]
Rawhide

[Supporting Documents]
#1. [Clint Eastwood]
  Clinton Eastwood Jr. (born May 31, 1930) is an American actor, filmmaker, musician, and politician.
  After achieving success in the Western TV series "Rawhide", he rose to international fame with his role as the Man with No Name in Italian filmmaker Sergio Leone's "Dollars" Trilogy of spaghetti Westerns during the 1960s and as antihero cop Harry Callahan in the five "Dirty Harry" films throughout the 1970s and 1980s.
  These roles, among others, have made Eastwood an enduring cultural icon of masculinity.
#2. [Pat Hingle]
  Martin Patterson Hingle (July 19, 1924 – January 3, 2009) was an American character actor who appeared in hundreds of television shows and feature films.
  His first film was "On the Waterfront" in 1954.
  He often played tough authority figures.
  Hingle was a close friend of Clint Eastwood and appeared in the Eastwood films "Hang 'em High", "The Gauntlet", and "Sudden Impact".

[Explanation]
Eastwood was [#1 Clint Eastwood : an American actor, filmmaker, musician] and [#1 Clint Eastwood : achieving success in the Western TV series "Rawhide"]. The next part to consider is whether Eastwood was a close friend Hingle. Hingle [#2 Pat Hingle : was a close friend of Clint Eastwood and appeared in the Eastwood films "Hang 'em High", "The Gauntlet", and "Sudden Impact".]. Hingle was a close friend of Eastwood, who achieved success in the Western TV series "Rawhide". So the answer is Rawhide.


[Question]
Ernest Foot was the best friend of the fighter pilot who had how many victories?

[Answer]
44

[Supporting Documents]
#1. [Ernest Foot]
  Major Ernest Leslie Foot (19 May 1895 – 23 June 1923) was an English World War I flying ace credited with five aerial victories.
  He was the best friend of Albert Ball.
#2. [Albert Ball]
  Albert Ball, (14 August 1896 – 7 May 1917) was an English fighter pilot during the First World War.
  At the time of his death he was the United Kingdom's leading flying ace, with 44 victories, and remained its fourth-highest scorer behind Edward Mannock, James McCudden, and George McElroy.

[Explanation]
Ernest Foot [#1 Ernest Foot : was the best friend of Albert Ball.]. Since Ernest Foot was the best friend of Albert Ball, the next step is to identify the number of victories Ball had. Ball was [#2 Albert Ball : the United Kingdom's leading flying ace, with 44 victories]. Foot was the best friend of Ball, who had 44 victories. So the answer is 44.


[Question]
A medieval fortress in Dirleton, East Lothian, Scotland borders on the south side of what coastal area?

[Answer]
Yellowcraig

[Supporting Documents]
#1. [Yellowcraigs]
  Yellowcraig, less commonly known as Broad Sands Bay, is a coastal area of forest, beach and grassland in East Lothian, south-east Scotland.
  Yellowcraig is partly within the Firth of Forth Site of Special Scientific Interest (SSSI).
  It is bordered to the north by the Firth of Forth, to the south by the village of Dirleton and Dirleton Castle, to the east by the North Berwick West Links golf course, and to the west by the Archerfield Estate and Links golf courses.
#2. [Dirleton Castle]
  Dirleton Castle is a medieval fortress in the village of Dirleton, East Lothian, Scotland.
  It lies around west of North Berwick, and around east of Edinburgh.
  The oldest parts of the castle date to the 13th century, and it was abandoned by the end of the 17th century.

[Explanation]
Dirleton Castle [#2 Dirleton Castle : is a medieval fortress in the village of Dirleton, East Lothian, Scotland.]. The next step is to identify what costal area Dirleton Castle borders on the south side of. Yellowcraig is borded [#1 Yellowcraigs : to the south by the village of Dirleton and Dirleton Castle]. Dirleton Castle is located south of Yellowcraig. So the answer is Yellowcraig.


[Question]
Are Random House Tower and 888 7th Avenue both used for real estate?

[Answer]
no

[Supporting Documents]
#1. [888 7th Avenue]
  888 7th Avenue is a 628 ft (191m) tall modern-style office skyscraper in Midtown Manhattan which was completed in 1969 and has 46 floors.
  Emery Roth & Sons designed the building, which is tied with Central Park Place for the 110th tallest building in New York.
  It currently carries the Vornado Realty Trust corporate headquarters.
  Previously known as the Arlen Building, its namesake being the company responsible for its construction, Arlen Realty & Development Corporation.
  The Red Eye Grill is located in the building at street level.
#2. [Penguin Random House Tower]
  The Penguin Random House Tower, also known as the Park Imperial Apartments, is a 52-story mixed-use tower in New York City, United States, that is used as the American headquarters of book publisher Penguin Random House and a luxury apartment complex.
  The PRH entrance is on Broadway and goes up to 27 floors, while the apartment complex entrance is on West 56th Street.
  Rising to 684 ft (208 m), it is the 77th tallest building in New York.

[Explanation]
The Random House Tower [#2 Penguin Random House Tower : is a 52-story mixed-use tower in New York City, United States, that is used as the American headquarters of book publisher Penguin Random House and a luxury apartment complex.]. 888 7th Avenue [#1 888 7th Avenue : carries the Vornado Realty Trust corporate headquarters]. The Random House Tower is used as the headquarters of book publisher Random House and a luxury apartment complex, while 888 7th Avenue carries the Vornado Realty Trust corporate headquarters. So the answer is no.
    \end{lstlisting}






